The Hidden Threat in Plain Text: Attacking RAG Data Loaders

Large Language Models (LLMs) have transformed human-machine interaction since ChatGPT's 2022 debut, with Retrieval-Augmented Generation (RAG) emerging as a key framework that enhances LLM outputs by integrating external knowledge. However, RAG's reliance on ingesting external documents introduces new vulnerabilities. This paper exposes a critical security gap at the data loading stage, where malicious actors can stealthily corrupt RAG pipelines by exploiting document ingestion. We propose a taxonomy of 9 knowledge-based poisoning attacks and introduce two novel threat vectors -- Content Obfuscation and Content Injection -- targeting common formats (DOCX, HTML, PDF). Using an automated toolkit implementing 19 stealthy injection techniques, we test five popular data loaders, finding a 74.4% attack success rate across 357 scenarios. We further validate these threats on six end-to-end RAG systems -- including white-box pipelines and black-box services like NotebookLM and OpenAI Assistants -- demonstrating high success rates and critical vulnerabilities that bypass filters and silently compromise output integrity. Our results emphasize the urgent need to secure the document ingestion process in RAG systems against covert content manipulations.

==> Tables/DOCX_pivot_colored.tex <==

\begin{tabular}{@{}ccccccccc@{}} \toprule
                           & \multicolumn{1}{c|}{}                 & \multicolumn{2}{c|}{\textbf{docling}}        & \multicolumn{1}{c|}{\textbf{haystack}} & \multicolumn{1}{c|}{\textbf{langchain}} & \multicolumn{2}{c|}{\textbf{llamaindex}}                         & \textbf{llmsherpa} \\
                           & \multicolumn{1}{c|}{}                 & DOCX & \multicolumn{1}{c|}{default} & \multicolumn{1}{c|}{docx}     & \multicolumn{1}{c|}{Docx2txt}  & llamaparse & \multicolumn{1}{c|}{simpleDirectoryReader} & default   \\ \midrule
\multicolumn{9}{c}{\textit{Content Obfuscation}}          \\ \midrule
Diacritical Marks      & \multicolumn{1}{c|}{mask1}            & \cellcolor{rgb:241,224,168} 0.41 & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}     & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}      & \cellcolor{rgb:241,224,168} 0.41       & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}                  & \cellcolor{rgb:241,224,168} 0.41      \\
Homoglyph Characters                  & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Reordering  Characters        & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 0.82 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 0.82}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 0.82}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 0.82}      & \cellcolor{rgb:144,238,144} 0.02       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 0.82}                  & \cellcolor{rgb:255,160,160} 0.82      \\
Zero-Width Characters                & \multicolumn{1}{c|}{mask1}            & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:144,238,144} 0.02       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Zero-Width Characters         & \multicolumn{1}{c|}{mask2}            & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:144,238,144} 0.01       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\ \midrule
\multicolumn{9}{c}{\textit{Context Injection}}                                                                                                                                                                                                              \\ \midrule
Out-of-Bound Text    & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Transparent Text & \multicolumn{1}{c|}{background-color} & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Transparent Text & \multicolumn{1}{c|}{vanish}           & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Zero-Size Font       & \multicolumn{1}{c|}{font1}            & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}      & \cellcolor{rgb:255,160,160} 0.99       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\ \bottomrule
\end{tabular}%
% \caption{PhantomPWN toolkit attack success rate at varying of techniques -- from both \textit{Semantic Corruption via Obfuscation} and\textit{Invisible Context Injection} families -- across different \textit{DOCX} data loader libraries and configurations. }
% \label{tab:DOCX}


==> Tables/HTML_pivot_colored.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \begin{table*}[!htpb]
% \label{tab:HTML}
% \centering
% \footnotesize
\begin{tabular}{@{}cccccccccc@{}} \toprule
                           & \multicolumn{1}{c|}{}                 & \multicolumn{2}{c|}{\textbf{docling}}        & \multicolumn{1}{c|}{\textbf{haystack}} & \multicolumn{2}{c|}{\textbf{langchain}}                 & \multicolumn{2}{c|}{\textbf{llamaindex}}                 & \textbf{llmsherpa} \\
                           & \multicolumn{1}{c|}{}                 & HTML & \multicolumn{1}{c|}{default} & \multicolumn{1}{c|}{html}     & BSHtml & \multicolumn{1}{c|}{UnstructuredHTML} & HTMLTagReader & \multicolumn{1}{c|}{llamaparse} & default   \\ \midrule
\multicolumn{10}{c}{\textit{Content Obfuscation}} \\ \midrule
Diacritical Marks     & \multicolumn{1}{c|}{mask1}            & \cellcolor{rgb:241,224,168} 0.42 & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.42}    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.42}     & \cellcolor{rgb:241,224,168} 0.42   & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.42}             & \cellcolor{rgb:241,224,168} 0.42          & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.51}       & \cellcolor{rgb:241,224,168} 0.42      \\
Font Poisoning             & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}       & \cellcolor{rgb:255,160,160} 1.00      \\
Homoglyph Characters                 & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}       & \cellcolor{rgb:255,160,160} 1.00      \\
Reordering Characters         & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 0.99}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.01}       & \cellcolor{rgb:255,160,160} 1.00      \\
Zero-Width Characters                & \multicolumn{1}{c|}{mask1}            & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.02}       & \cellcolor{rgb:255,160,160} 1.00      \\
Zero-Width Characters                & \multicolumn{1}{c|}{mask2}            & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.02}       & \cellcolor{rgb:255,160,160} 1.00      \\ \midrule
\multicolumn{10}{c}{\textit{Context Injection}}                              \\ \midrule
Camouflage Element & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:245,183,177} 0.60}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Metadata         & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:144,238,144} 0.00 & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:144,238,144} 0.00   & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}             & \cellcolor{rgb:144,238,144} 0.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Out-of-Bound Text    & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:255,160,160} 1.00      \\
Transparent Text & \multicolumn{1}{c|}{background-color} & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:245,183,177} 0.62}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Transparent Text & \multicolumn{1}{c|}{opacity00}        & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:245,183,177} 0.66}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Transparent Text & \multicolumn{1}{c|}{opacity01}        & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.43}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Zero-Size Font       & \multicolumn{1}{c|}{font00}           & \cellcolor{rgb:144,238,144} 0.00 & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.54}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Zero-Size Font   & \multicolumn{1}{c|}{font01}           & \cellcolor{rgb:144,238,144} 0.00 & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.52}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 0.99}       & \cellcolor{rgb:144,238,144} 0.00      \\
Zero-Size Font       & \multicolumn{1}{c|}{scaling}          & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.49}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}       & \cellcolor{rgb:144,238,144} 0.00      \\
Zero-Size Font       & \multicolumn{1}{c|}{visibilityHidden} & \cellcolor{rgb:255,160,160} 1.00 & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}    & \multicolumn{1}{c|}{\cellcolor{rgb:194,230,153} 0.39}     & \cellcolor{rgb:255,160,160} 1.00   & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}             & \cellcolor{rgb:255,160,160} 1.00          & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}       & \cellcolor{rgb:144,238,144} 0.00 \\ \bottomrule
\end{tabular}% 
% \caption{PhantomPWN toolkit attack success rate at varying of techniques -- from both \textit{Semantic Corruption via Obfuscation} and \textit{Invisible Context Injection} families -- across different \textit{HTML} data loader libraries and configurations. }
% \end{table*}

==> Tables/PDF_pivot_colored.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[!htpb]\label{tab:pdf}
% \centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccc@{}}  \toprule
                           & \multicolumn{1}{c|}{}                 & \multicolumn{2}{c|}{\textbf{docling}}            & \multicolumn{2}{c|}{\textbf{haystack}}         & \multicolumn{4}{c|}{\textbf{langchain}}                                & \multicolumn{2}{c|}{\textbf{llamaindex}}                         & \textbf{llmsherpa} \\
                           & \multicolumn{1}{c|}{}                 & default & \multicolumn{1}{c|}{pyPDFium} & PDFMiner & \multicolumn{1}{c|}{pyPDF} & PDFPlumber & PyMUPDF & PyPDFium2 & \multicolumn{1}{c|}{pyPDF} & llamaparse & \multicolumn{1}{c|}{simpleDirectoryReader} & default   \\ \midrule
\multicolumn{13}{c}{\textit{Content Obfuscation}}                                                                                                                                                                                                                                                      \\ \midrule
Diacritical Marks     & \multicolumn{1}{c|}{mask1}            & \cellcolor{rgb:241,224,168} 0.41    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}     & \cellcolor{rgb:241,224,168} 0.41     & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}  & \cellcolor{rgb:241,224,168} 0.41       & \cellcolor{rgb:241,224,168} 0.41    & \cellcolor{rgb:241,224,168} 0.41      & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}  & \cellcolor{rgb:241,224,168} 0.41       & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.41}                  & \cellcolor{rgb:245,183,177} 0.74      \\
Font Poisoning             & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:255,160,160} 1.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Homoglyph Characters                 & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 1.00    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:255,160,160} 1.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Reordering Characters         & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:255,160,160} 0.97    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.03}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 0.96       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:144,238,144} 0.02      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:144,238,144} 0.02       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Zero-Width Characters                & \multicolumn{1}{c|}{mask1}            & \cellcolor{rgb:245,183,177} 0.72    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 0.99      \\
Zero-Width Characters                & \multicolumn{1}{c|}{mask2}            & \cellcolor{rgb:245,183,177} 0.74    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\ \midrule
\multicolumn{13}{c}{\textit{Content Injection}}                                                                                                                                                                                                                                                        \\ \midrule
Camouflage Element& \multicolumn{1}{c|}{default}          & \cellcolor{rgb:241,224,168} 0.51    & \multicolumn{1}{c|}{\cellcolor{rgb:241,224,168} 0.48}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:255,160,160} 1.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 0.98       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Metadata         & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:144,238,144} 0.00    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:144,238,144} 0.00     & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}                  & \cellcolor{rgb:144,238,144} 0.00      \\
Out-of-Bound Text    & \multicolumn{1}{c|}{default}          & \cellcolor{rgb:144,238,144} 0.00    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:144,238,144} 0.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 0.99      \\
Transparent Text & \multicolumn{1}{c|}{background-color} & \cellcolor{rgb:255,160,160} 1.00    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:255,160,160} 1.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Transparent Text & \multicolumn{1}{c|}{opacity00}        & \cellcolor{rgb:255,160,160} 1.00    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:255,160,160} 1.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Transparent Text & \multicolumn{1}{c|}{opacity01}        & \cellcolor{rgb:255,160,160} 1.00    & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:255,160,160} 1.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:255,160,160} 1.00      \\
Zero-Size Font       & \multicolumn{1}{c|}{font00}           & \cellcolor{rgb:144,238,144} 0.00    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:144,238,144} 0.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:144,238,144} 0.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:144,238,144} 0.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:144,238,144} 0.00      \\
Zero-Size Font       & \multicolumn{1}{c|}{font01}           & \cellcolor{rgb:144,238,144} 0.13    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:144,238,144} 0.00      \\
Zero-Size Font        & \multicolumn{1}{c|}{scaling}          & \cellcolor{rgb:144,238,144} 0.13    & \multicolumn{1}{c|}{\cellcolor{rgb:144,238,144} 0.00}     & \cellcolor{rgb:255,160,160} 1.00     & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \cellcolor{rgb:255,160,160} 1.00    & \cellcolor{rgb:144,238,144} 0.00      & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}  & \cellcolor{rgb:255,160,160} 1.00       & \multicolumn{1}{c|}{\cellcolor{rgb:255,160,160} 1.00}                  & \cellcolor{rgb:144,238,144} 0.00 \\ \bottomrule
\end{tabular}%
% }
% \caption{PhantomPWN toolkit attack success rate at varying of techniques -- from both \textit{Semantic Corruption via Obfuscation} and \textit{Invisible Context Injection} families -- across different \textit{PDF} data loader libraries and configurations. }
% \end{table*}

==> Tables/exp2-tab.tex <==
\begin{table*}[!htpb]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{ll|ccc|ccc}
\toprule
\multicolumn{2}{c|}{} & \multicolumn{3}{c|}{\textbf{White-box}} & \multicolumn{3}{c}{\textbf{Black-box}} \\ 
 &  & deepseek-r1 & gemma3 & gpt-4o & llama3 & notebooklm & o3-mini \\
\midrule
Camouflage Element & default & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Diacritical Marks& mask1 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{247,198,165} 7/10 & \cellcolor[RGB]{247,198,165} 7/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{144,238,144} 0/10 \\
Font Poisoning  & default & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Homoglyph Characters& default & \cellcolor[RGB]{163,235,149} 1/10 & \cellcolor[RGB]{247,198,165} 7/10 & \cellcolor[RGB]{249,186,163} 8/10 & \cellcolor[RGB]{183,232,154} 2/10 & \cellcolor[RGB]{163,235,149} 1/10 & \cellcolor[RGB]{144,238,144} 0/10 \\
Metadata & default & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{144,238,144} 0/10 \\
Out-of-Bound Text& default & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Reordering Characters& default & \cellcolor[RGB]{252,173,162} 9/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{252,173,162} 9/10 \\
Transparent Text & background-color & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Transparent Text & opacity00 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Transparent Text & opacity01 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Zero-Size Font & font00 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{252,173,162} 9/10 \\
Zero-Size Font & font01 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 \\
Zero-Size Font& scaling & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{252,173,162} 9/10 \\
Zero-Width Characters & mask3 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{144,238,144} 0/10 & \cellcolor[RGB]{255,160,160} 10/10 & \cellcolor[RGB]{183,232,154} 2/10 \\
\bottomrule
\end{tabular}%
}
\caption{{\textit{Experiment 2 -- End-to-End RAG Manipulation.} Attack success rate at varying of PDF techniques across different RAG systems.}}
\label{tab:exp2}
\end{table*}


==> Tables/ocr_pivot_colored.tex <==
% \begin{table}[!htpb]\label{tab:OCR}
% \footnotesize
\begin{tabular}{cc|c|c|c} \toprule
              &         & docling   & langchain                & langchain        \\
              &         & tesseract & PyMuPDFLoader\_tesseract & pyPDF\_tesseract \\ \hline
OCR-Poisoning & default & \cellcolor{rgb:255,160,160} 1.00      & \cellcolor{rgb:255,160,160} 1.00                     & \cellcolor{rgb:255,160,160} 1.00 \\ \bottomrule
\end{tabular}
% \caption{OCR}
% \end{table}
